A Spatio-Temporal Representation Learning as an Alternative to Traditional Glosses in Sign Language Translation and Production

This work addresses the challenges associated with the use of glosses in both Sign Language Translation (SLT) and Sign Language Production (SLP). While glosses have long been used as a bridge between sign language and spoken language, they come with two major limitations that impede the advancement of sign language systems. First, annotating the glosses is a labor-intensive and time-consuming process, which limits the scalability of datasets. Second, the glosses oversimplify sign language by stripping away its spatio-temporal dynamics, reducing complex signs to basic labels and missing the subtle movements essential for precise interpretation. To address these limitations, we introduce Universal Gloss-level Representation (UniGloR), a framework designed to capture the spatio-temporal features inherent in sign language, providing a more dynamic and detailed alternative to the use of the glosses. The core idea of UniGloR is simple yet effective: We derive dense spatio-temporal representations from sign keypoint sequences using self-supervised learning and seamlessly integrate them into SLT and SLP tasks. Our experiments in a keypoint-based setting demonstrate that UniGloR either outperforms or matches the performance of previous SLT and SLP methods on two widely-used datasets: PHOENIX14T and How2Sign.

==> tab/ablation.tex <==
\begin{table}[b]
\scriptsize
\centering
\caption{The results of additional ablation study. P, H, and N denote PHOENIX14T, How2Sign, and NIASL21, respectively.}\label{tab:additional-ablation}
\vspace{-1em}
\begin{minipage}{0.30\linewidth}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cc} \toprule
Decoding Type &B@4 &R@L\\ \midrule
 AR &10.42 	&26.66  \\
 NAR (ours) &\textbf{11.01}	&\textbf{27.03} \\ \bottomrule
\end{tabular}%
}
\end{minipage}
\hfill
\begin{minipage}{0.30\linewidth}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cc} \toprule
Pooling Type &B@4 &R@L\\ \midrule
 Mean &\textbf{11.12} 	&\textbf{27.47} \\
 CLS (ours) &11.01	&27.03 \\ \bottomrule
\end{tabular}%
}
\end{minipage}
\hfill
\begin{minipage}{0.30\linewidth}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cc} \toprule
Window Size &B@4 &R@L\\ \midrule
 N=32 &8.59 	&23.10 \\
 N=64 &8.15 	&22.32 \\ \midrule
 N=15 (ours) &\textbf{11.01}	&\textbf{27.03} \\ \bottomrule
\end{tabular}%
}
\end{minipage}
\vspace{-1em}
\end{table}

==> tab/frame-stats.tex <==
\begin{table}[t]
    % \scriptsize
    \centering
    \caption{Statistics of Sign Language Datasets, including various subsets of NIASL2021. This provides an in-depth overview of the datasets used in this study. Additionally, it presents the maximum, minimum, and average numbers of frames (NoF) for each dataset, offering insights into the range and complexity of the data.}\label{tab:frame-stats}
    \resizebox{0.6\linewidth}{!}{%
    \begin{tabular}{l|c|c|c|c} \toprule 
         Dataset& Train / Valid / Test&Max NoF&  Min NoF&  Avg NoF\\ \midrule 
         PHOENIX14T~\cite{camgoz2018neural}& 7,096 / 519 / 642&475 &  16 &  116 \\  
         How2Sign~\cite{duarte2021how2sign} & 31,128 / 1,741 / 2,322&2,579 &  32  &  173 \\  
         NIASL2021~\cite{huerta2022kosign}& 160,644 / 10,079 / 9,989&1,887&  37&  466\\ \bottomrule \toprule
 NIASL2021 (5\%)& 3,361 / 215 / 193& 221& 37&188
\\
 NIASL2021 (10\%)& 14,038 / 865 / 877& 275& 37&231
\\
 NIASL2021 (50\%)& 93,851 / 5,966 / 5,865& 466& 37&372\\ \bottomrule
    \end{tabular}
    }
\end{table}

% \begin{table}
%     \scriptsize
%     \centering
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l|c|c|c|c} \toprule 
%          & Train / Valid / Test&Max NoF&  Min NoF&  Avg NoF\\ \midrule 
%          PDF (0.05)& 3,361 / 215 / 193&221&  37&  188\\  
%          PDF (0.1)& 14,038 / 865 / 877&275&  37&  231\\  
%          PDF (0.5)& 93,851 / 5,966 / 5,865&466&  37&  372\\ \bottomrule
%     \end{tabular}
%     }
%     \caption{Statistics of Sign Language Datasets. NoF means number of frames.}
%     \label{tab:PDF}
% \end{table}



==> tab/nia_subset_slp_res.tex <==
\begin{figure}[t]
    \centering
    \scriptsize
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lcccccc} \toprule 
         Dataset Subset& BLEU-1& BLEU-2& BLEU-3& BLEU-4& ROUGE \\ \midrule 
         NIASL2021 (5\%)& 24.01& 16.61& 10.71& 7.16& 23.83 \\  
         NIASL2021 (10\%)& 11.42& 7.48& 3.75& 1.47& 11.79 \\  
         NIASL2021 (50\%)& 8.97& 5.25& 3.09& 1.31& 10.05 \\ 
        NIASL2021 (100\%)& 5.41& 2.48& 1.03& 0.42& 6.02 \\ \bottomrule
    \end{tabular}
    }
    \caption{SLP Performance Across Length Subsets: \% corresponds to the initial 5\%, 10\%, and 50\% segments of the PDF distribution.}\label{tab:nia_subset_slp_res}
\end{figure}

==> tab/slp-gloss.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\scriptsize
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|cccccc} \toprule
SLP Models& B@1& B@2& B@3& B@4&R@L& MPJPE$\downarrow$\\ \midrule
\rowcolor{gray!40}
 \multicolumn{7}{c}{RWTH-PHOENIX-WEATHER-2014T}\\ \midrule
PT$^\ddagger$~\cite{saunders2020progressive}&        14.84&        8.00&        5.49&        4.19&12.83&         0.590\\
NSLP-G~\cite{hwang2021non} &        18.25&        11.06&        7.86&        6.14&17.71&         0.332\\ \bottomrule \toprule
 UniGloR-SLP (Ours)& \textbf{29.60}& \textbf{21.25}& \textbf{16.48}& \textbf{13.44}&\textbf{31.38}&\textbf{0.183}\\ \midrule
 \rowcolor{gray!40}
 \multicolumn{7}{c}{NIASL2021}\\ \midrule
 PT$^\ddagger$~\cite{saunders2020progressive}& 1.53& 0.54& 0.25& 0.07& 1.85&0.407\\
 NSLP-G~\cite{hwang2021non} & 4.17& 1.82& 0.89& 0.36& 4.26&0.453\\ \bottomrule \toprule
 UniGloR-SLP (Ours)& \textbf{5.41}& \textbf{2.48}& \textbf{1.03}& \textbf{0.42}& \textbf{6.02}&\textbf{0.448}\\ \bottomrule
\end{tabular}%
}
\caption{Production results on PHOENIX14T and NIASL2021 with gloss-based methods.}
\label{tab:slp-results-gloss}
\vspace{-1.3em}
\end{table}

==> tab/slt-gloss.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
    \scriptsize
    \centering
    \begin{subtable}{\linewidth}
        \resizebox{\linewidth}{!}{%
        \begin{tabular}{l|ccccc} \toprule
        SLT Models& B@1 & B@2 & B@3 & B@4 & R@L \\ \midrule
        \rowcolor{gray!40}
         \multicolumn{6}{c}{RWTH-PHOENIX-WEATHER-2014T}\\ \midrule
        Joint-SLT$^\star$~\cite{camgoz2020sign}&        24.88 &        15.98 &        11.66 &        9.28 &         24.76
        \\
        SLTUNET$^\star$~\cite{zhang2023sltunet}&        25.34&        17.24&        13.02&        10.63&         25.56\\ \bottomrule \toprule
         UniGloR-SLT (Ours)& \textbf{26.68} & \textbf{ 18.22} & \textbf{ 13.73} & \textbf{11.01} &\textbf{27.03}\\ \midrule 
         \rowcolor{gray!40}
         \multicolumn{6}{c}{NIASL2021}\\ \midrule
         Joint-SLT$^\star$~\cite{camgoz2020sign}
        & \textbf{53.27}& \textbf{43.92}& \textbf{37.22}& \textbf{32.16}&\textbf{52.91}\\
         SLTUNET$^\star$~\cite{zhang2023sltunet}& 52.36& 43.03& 36.39& 31.39&52.07\\ \bottomrule \toprule
         UniGloR-SLT (Ours)& 49.49& 39.68& 32.80& 27.69&48.81\\ \bottomrule
        \end{tabular}%
        }
        \caption{Translation Performance}\label{tab:slt-results-gloss}
    \end{subtable}
\hfill
    \begin{subtable}{\linewidth}
        \resizebox{\linewidth}{!}{%
        \begin{tabular}{l|cccccc} \toprule
        SLP Models& B@1& B@2& B@3& B@4&R@L& MPJPE$\downarrow$\\ \midrule
        \rowcolor{gray!40}
         \multicolumn{7}{c}{RWTH-PHOENIX-WEATHER-2014T}\\ \midrule
        PT$^\ddagger$~\cite{saunders2020progressive}&        14.84&        8.00&        5.49&        4.19&12.83&         0.590\\
        NSLP-G~\cite{hwang2021non} &        18.25&        11.06&        7.86&        6.14&17.71&         0.332\\ \bottomrule \toprule
         UniGloR-SLP (Ours)& \textbf{29.60}& \textbf{21.25}& \textbf{16.48}& \textbf{13.44}&\textbf{31.38}&\textbf{0.183}\\ \midrule
         \rowcolor{gray!40}
         \multicolumn{7}{c}{NIASL2021}\\ \midrule
         PT$^\ddagger$~\cite{saunders2020progressive}& 1.53& 0.54& 0.25& 0.07& 1.85&0.407\\
         NSLP-G~\cite{hwang2021non} & 4.17& 1.82& 0.89& 0.36& 4.26&0.453\\ \bottomrule \toprule
         UniGloR-SLP (Ours)& \textbf{5.41}& \textbf{2.48}& \textbf{1.03}& \textbf{0.42}& \textbf{6.02}&\textbf{0.448}\\ \bottomrule
        \end{tabular}%
        }
        \caption{Production Performance}\label{tab:slp-results-gloss}
    \end{subtable}
    \caption{Performance comparison on PHOENIX14T and NIASL2021 with gloss-based methods. We exclude How2Sign due to the absence of glosses.}
\end{table}

% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table}[]
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{l|ccccc} \toprule
% SLT Models& B@1 & B@2 & B@3 & B@4 & R@L \\ \midrule
%  \multicolumn{6}{c}{Gloss-based}\\ \midrule
% Joint-SLT$^\star$~\cite{camgoz2020sign}&        &        &        &        &         \\
% SLTUNET$^\star$~\cite{zhang2023sltunet}&        &        &        &        &         \\ \midrule 
%  \multicolumn{6}{c}{Gloss-free}\\ \midrule
%  CTR-GCN~\cite{chen2021channel}                                      & 46.15& 36.43& 29.70& 24.97&45.96\\
%  CTR-GCN~\cite{chen2021channel} + MS-TCN~\cite{liu2020disentangling}& 46.74& 37.09& 30.39& 25.50&46.53\\
%  Joint-SLT$^{\dagger\star}$~\cite{camgoz2020sign}& 45.61& 36.08& 29.58& 24.84&45.45\\
%  ConSLT$^\star$~\cite{10095466}& 46.50& 37.00& 30.51& 25.78&46.24\\ \bottomrule \toprule
%  UniGloR-SLT (Ours)& \textbf{49.49}& \textbf{39.68}& \textbf{32.80}& \textbf{27.69}&\textbf{48.81}\\ \bottomrule
% \end{tabular}%
% }
% \caption{Performance Comparison with Gloss-based Methods on PHOENIX14T.}
% \label{tab:slt-results-gloss}
% \end{table}

==> tab/slt-sota.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\scriptsize
\centering
    \begin{subtable}[b]{\linewidth}
        \resizebox{\linewidth}{!}{%
        \begin{tabular}{l|ccccc} \toprule
        SLT Models& B@1& B@2& B@3& B@4& R@L\\ \midrule
        \rowcolor{gray!40}
         \multicolumn{6}{c}{RWTH-PHOENIX-WEATHER-2014T}\\ \midrule
        CTR-GCN~\cite{chen2021channel}                                      &        22.41 &        14.57 &        10.82 &        8.66 &         22.10\\
        CTR-GCN~\cite{chen2021channel} + MS-TCN~\cite{liu2020disentangling}&        22.10 &        14.51 &        10.70 &        8.62 &         21.82\\
        Joint-SLT$^{\dagger\star}$~\cite{camgoz2020sign}&        21.31 &        14.17 &        10.05 &        8.12 &         22.56\\
         ConSLT$^\star$~\cite{10095466}& 21.09 & 13.93 & 10.48 & 8.49 &21.81\\ \bottomrule \toprule
        UniGloR-SLT (Ours)&        \textbf{26.68} &       \textbf{ 18.22} &       \textbf{ 13.73} &        \textbf{11.01} &         \textbf{27.03}\\ \midrule
        \rowcolor{gray!40}
         \multicolumn{6}{c}{How2Sign}\\ \midrule
         CTR-GCN~\cite{chen2021channel}                                      & 13.81& 5.51& 2.42& 0.88&10.81
        \\
         CTR-GCN~\cite{chen2021channel} + MS-TCN~\cite{liu2020disentangling}& 13.33& 5.70& 2.61& 1.00&11.03
        \\
         Joint-SLT$^{\dagger\star}$~\cite{camgoz2020sign}& 11.11& 4.41& 1.98& 0.78&10.61
        \\
         ConSLT$^\star$~\cite{10095466}& 12.06& 4.75& 1.92& 0.84&9.72\\ \bottomrule \toprule
         UniGloR-SLT (Ours)& \textbf{14.26}& \textbf{5.99}& \textbf{2.96}& \textbf{1.47}&\textbf{11.05}\\ \midrule
         \rowcolor{gray!40}
         \multicolumn{6}{c}{NIASL2021}\\ \midrule
         CTR-GCN~\cite{chen2021channel}                                      & 46.15& 36.43& 29.70& 24.97&45.96
        \\
         CTR-GCN~\cite{chen2021channel} + MS-TCN~\cite{liu2020disentangling}& 46.74& 37.09& 30.39& 25.50&46.53
        \\
         Joint-SLT$^{\dagger\star}$~\cite{camgoz2020sign}& 45.61& 36.08& 29.58& 24.84&45.45
        \\
         ConSLT$^\star$~\cite{10095466}& 46.50& 37.00& 30.51& 25.78&46.24\\ \bottomrule \toprule
         UniGloR-SLT (Ours)& \textbf{49.49}& \textbf{39.68}& \textbf{32.80}& \textbf{27.69}&\textbf{48.81}\\ \bottomrule
        \end{tabular}%
        }
        \caption{Translation performance}\label{tab:slt-results}
    \end{subtable}
    \vfill
    \begin{subtable}[b]{\linewidth}
        \resizebox{\linewidth}{!}{%
        \begin{tabular}{l|cccccc} \toprule
        SLP Models& B@1& B@2& B@3& B@4& R@L &MPJPE$\downarrow$\\ \midrule
        \rowcolor{gray!40}
         \multicolumn{7}{c}{RWTH-PHOENIX-WEATHER-2014T}\\ \midrule
        PT$^\ddagger$~\cite{saunders2020progressive}
        &        12.07&        5.94&        4.04&        3.08&         11.06&0.602\\
        NSLP-G~\cite{hwang2021non} 
        &        19.10&        12.10&        8.87&        6.97&         18.62&0.335\\ \bottomrule \toprule
        UniGloR-SLP (Ours)&        \textbf{29.60}&       \textbf{21.25}&       \textbf{16.48}&        \textbf{13.44}&         \textbf{31.38}&\textbf{0.183}\\ \midrule
        \rowcolor{gray!40}
         \multicolumn{7}{c}{How2Sign}\\ \midrule
         PT$^\ddagger$~\cite{saunders2020progressive}
        & 11.88& 4.50& 1.75& 0.42& 9.76&0.466\\
         NSLP-G~\cite{hwang2021non} 
        & 9.73& 3.67& 1.53& 0.48& 10.18&0.427\\ \bottomrule \toprule
         UniGloR-SLP (Ours)& \textbf{12.69}& \textbf{5.12}& \textbf{2.36}& \textbf{1.06}& \textbf{10.93}&\textbf{0.169}\\ \midrule
         \rowcolor{gray!40}
         \multicolumn{7}{c}{NIASL2021}\\ \midrule
         PT$^\ddagger$~\cite{saunders2020progressive}
        & 0.87& 0.42& 0.22& 0.10& 0.99&0.521\\
         NSLP-G~\cite{hwang2021non} 
        & 3.17& 1.04& 0.39& 0.13& 3.22&0.464\\ \bottomrule \toprule
         UniGloR-SLP (Ours)& \textbf{5.41}& \textbf{2.48}& \textbf{1.03}& \textbf{0.42}& \textbf{6.02}&\textbf{0.448}\\ \bottomrule
        \end{tabular}%
        }
        \caption{Production performance}
        \label{tab:slp-results}
    \end{subtable}
    \caption{Performance comparison on PHOENIX14T, How2Sign, and NIASL2021. B@N and R@L denote the BLEU-N, and ROUGE- L scores, respectively. We reproduced most baselines due to the different modality of nature (RGB vs. keypoints). $\star$ denotes modification to accept keypoints as input. $\dagger$ denotes results reproduced under the gloss-free setting. $\ddagger$ denotes results reproduced without ground-truth. The best results are highlighted in bold.}
    \vspace{-0.3em}
\end{table}

==> tab/spec.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\scriptsize
\centering
\caption{Model size comparison. We provide a detailed overview of the model sizes for both SLT and SLP models, including the number of trainable parameters, total parameters and the overall model size in megabytes. $\star$ denotes modification to accept keypoints as input. $\dagger$ denotes results reproduced under the gloss-free setting. $\ddagger$ denotes results reproduced without ground-truth.} \label{tab:model-spec}
\resizebox{0.6\linewidth}{!}{%
\begin{tabular}{l|ccc} \toprule
\multirow{2}{*}{Models}& Trainable&Total& Model\\
 & Parameter& Parameter&Size\\ \midrule
\rowcolor{gray!40}
\multicolumn{4}{c}{SLT Models}\\ \midrule
CTR-GCN~\cite{chen2021channel}                                      &        31.4 M &31.4 M &        62.8 MB\\
CTR-GCN~\cite{chen2021channel} + MS-TCN~\cite{liu2020disentangling}&        31.9 M &31.9 M &        63.7 MB\\
Joint-SLT$^{\dagger\star}$~\cite{camgoz2020sign}&        30.2 M &30.2 M &        60.5 MB\\
 ConSLT$^\star$~\cite{10095466}& 30.2 M &30.2 M & 60.5 MB\\
 Joint-SLT$^{\star}$~\cite{camgoz2020sign}& 34.3 M &34.3 M &68.6 MB\\
  SLTUNET$^\star$~\cite{zhang2023sltunet}& 34.5 M &34.5 M &68.6 MB\\
UniGloR-SLT (Ours)&        30.4 M &52.9 M&       105.8 MB\\ \midrule
\rowcolor{gray!40}
\multicolumn{4}{c}{SLP Models}\\ \midrule
 PT$^\ddagger$~\cite{saunders2020progressive}& 26.3 M &26.3 M & 52.5 MB\\ 
 NSLP-G~\cite{hwang2021non}& 34.8 M &34.8 M & 54.8 MB\\
 UniGloR-SLP (Ours)& 87.8 M&245 M& 490.1 MB\\ \bottomrule
\end{tabular}%
}
% \vspace{-1.5em}
\end{table}
